CLASS Survey Description: Coronal Line Needles in the SDSS Haystack

Coronal lines are a powerful, yet poorly understood, tool to identify and characterize Active Galactic Nuclei (AGNs). There have been few large scale surveys of coronal lines in the general galaxy population in the literature so far. Using a novel pre-selection technique with a flux-to-RMS ratio $F$, followed by Markov-Chain Monte Carlo (MCMC) fitting, we searched for the full suite of 20 coronal lines in the optical spectra of almost 1 million galaxies from the Sloan Digital Sky Survey (SDSS) Data Release 8. We present a catalog of the emission line parameters for the resulting 258 galaxies with detections. The Coronal Line Activity Spectroscopic Survey (CLASS) includes line properties, host galaxy properties, and selection criteria for all galaxies in which at least one line is detected. This comprehensive study reveals that a significant fraction of coronal line activity is missed in past surveys based on a more limited set of coronal lines; $\sim$60% of our sample do not display the more widely surveyed [Fe X] $\lambda$6374. In addition, we discover a strong correlation between coronal line and WISE W2 luminosities, suggesting that the mid-infrared flux can be used to predict coronal line fluxes. For each line we also provide a confidence level that the line is present, generated by a novel neural network, trained on fully simulated data. We find that after training the network to detect individual lines using 100,000 simulated spectra, we achieve an overall true positive rate of 75.49% and a false positive rate of only 3.96%.

==> column_descriptions.tex <==
\startlongtable
\begin{deluxetable*}{lp{7cm}llc}
% \tabletypesize{\footnotesize}
\label{tab:column_descriptions}
\tablecaption{Column descriptions for the CLASS catalog CSV file.}
\tablehead{\colhead{Column Name} & \colhead{Description} & \colhead{Units} & \colhead{Data Type} & \colhead{Source}}
\decimals
\startdata
SPECOBJID & SDSS Spec Object ID & & 64-bit integer & 2 \\
PLATE & SDSS Plate Number & & integer & 2 \\
MJD & SDSS Modified Julian Date of observation & MJD & integer & 2 \\
FIBERID & SDSS Fiber ID & & integer & 2 \\
ALLWISE\_SOURCEID & AllWISE Source ID & & string & 4 \\
ALLWISE\_COADDID & AllWISE Coadd ID & & string & 4 \\
RA & Right ascension & degrees & float & 2 \\
DEC & Declination & degrees & float & 2 \\
Z & Cosmological redshift & & float & 3 \\
Z\_ERR & Error in cosmological redshift & & float & 3 \\
N\_CL\_DETECT & Number of coronal lines detected in the spectrum & & integer & 1\\
LGM\_TOT\_P50 & Stellar mass median estimate from model photometry & $\log(M/M_\odot)$ & float & 3 \\
SFR\_TOT\_P50 & Star formation rate median estimate from model photometry & $\log($SFR$/M_\odot {\rm yr}^{-1})$ & float & 3 \\
V\_DISP & Stellar velocity dispersion & km s$^{-1}$ & float & 3 \\
V\_DISP\_ERR & Error in stellar velocity dispersion & km s$^{-1}$ & float & 3 \\
D4000 & 4000 \AA\ break from \citet{1983ApJ...273..105B} & & float & 3 \\
D4000\_ERR & Error in the 4000 \AA\ break from \citet{1983ApJ...273..105B} & & float & 3 \\
NII\_HALPHA & The flux ratio of [\ion{N}{2}] and H$\alpha$ & $\log($[\ion{N}{2}]$/$H$\alpha)$ & float & 3 \\
OIII\_HBETA & The flux ratio of [\ion{O}{3}] and H$\beta$ & $\log($[\ion{O}{3}]$/$H$\beta)$ & float & 3 \\
W1MPRO & WISE 1 profile-fit magnitude & mag & float & 4 \\
W2MPRO & WISE 2 profile-fit magnitude & mag & float & 4 \\
W3MPRO & WISE 3 profile-fit magnitude & mag & float & 4 \\
W4MPRO & WISE 4 profile-fit magnitude & mag & float & 4 \\
W1SIGMPRO & Error in WISE 1 profile-fit magnitude & mag & float & 4 \\
W2SIGMPRO & Error in WISE 2 profile-fit magnitude & mag & float & 4 \\
W3SIGMPRO & Error in WISE 3 profile-fit magnitude & mag & float & 4 \\
W4SIGMPRO & Error in WISE 4 profile-fit magnitude & mag & float & 4 \\
W12 & WISE 1 $-$ WISE 2 color & mag & float & 4 \\
W23 & WISE 2 $-$ WISE 3 color & mag & float & 4 \\
W12\_ERR & Error in WISE 1 $-$ WISE 2 color & mag & float & 4 \\
W23\_ERR & Error in WISE 2 $-$ WISE 3 color & mag & float & 4 \\
K01AGN & \citet{2001ApJ...556..121K} BPT AGN classification &  & boolean & 3 \\
K03AGN & \citet{2003MNRAS.346.1055K} BPT AGN classification & & boolean & 3 \\
JARRETTAGN & \citet{2011ApJ...735..112J} WISE AGN classification & & boolean & 4 \\
V\_OFF\_BALMER & Velocity offset of the Balmer lines & km s$^{-1}$ & float & 3 \\
V\_OFF\_BALMER\_ERR & Error in velocity offset of the Balmer lines & km s$^{-1}$ & float & 3 \\
V\_OFF\_FORBIDDEN & Velocity offset of forbidden lines & km s$^{-1}$ & float & 3 \\
V\_OFF\_FORBIDDEN\_ERR & Error in velocity offset of forbidden lines & km s$^{-1}$ & float & 3 \\
SERSIC\_N & S\'ersic index from $r$-band fit & & float & 5 \\
SERSIC\_TH50 & S\'ersic half-light radius along major axis & arcsec & float & 5 \\
ELPETRO\_TH50\_R & Elliptical Petrosian half-light radius in $r$-band & arcsec & float & 5 \\
U\_MAG & SDSS $u'$ magnitude & mag & float & 5 \\
G\_MAG & SDSS $g'$ magnitude & mag & float & 5 \\
R\_MAG & SDSS $r'$ magnitude & mag & float & 5 \\
I\_MAG & SDSS $i'$ magnitude & mag & float & 5 \\
Z\_MAG & SDSS $z'$ magnitude & mag & float & 5 \\
FEXI\_7982\_LOGL & Luminosity of the [\ion{Fe}{11}] $\lambda$7892 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEXI\_7982\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{11}] $\lambda$7892 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEXI\_7982\_FWHM & FWHM of the [\ion{Fe}{11}] $\lambda$7892 coronal line & km s$^{-1}$ & float & 1 \\
FEXI\_7982\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{11}] $\lambda$7892 coronal line & km s$^{-1}$ & float & 1 \\
FEXI\_7982\_VOFF & Velocity offset of the [\ion{Fe}{11}] $\lambda$7892 coronal line & km s$^{-1}$ & float & 1 \\
FEXI\_7982\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{11}] $\lambda$7892 coronal line & km s$^{-1}$ & float & 1 \\
FEXI\_7892\_EQW & Equivalent width of the [\ion{Fe}{11}] $\lambda$7892 coronal line & \AA\ & float & 1 \\
FEXI\_7892\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{11}] $\lambda$7892 coronal line & \AA\ & float & 1 \\
FEXI\_7892\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{11}] $\lambda$7892 coronal line & & float & 1 \\
FEXI\_7892\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{11}] $\lambda$7892 coronal line & & integer & 1 \\
FEXI\_7892\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{11}] $\lambda$7892 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEXI\_7892\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{11}] $\lambda$7892 line is present. & & float & 1 \\
SXII\_7609\_LOGL & Luminosity of the [\ion{S}{12}] $\lambda$7609 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
SXII\_7609\_LOGL\_ERR & Error in the luminosity of the [\ion{S}{12}] $\lambda$7609 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
SXII\_7609\_FWHM & FWHM of the [\ion{S}{12}] $\lambda$7609 coronal line & km s$^{-1}$ & float & 1 \\
SXII\_7609\_FWHM\_ERR & Error in the FWHM of the [\ion{S}{12}] $\lambda$7609 coronal line & km s$^{-1}$ & float & 1 \\
SXII\_7609\_VOFF & Velocity offset of the [\ion{S}{12}] $\lambda$7609 coronal line & km s$^{-1}$ & float & 1 \\
SXII\_7609\_VOFF\_ERR & Error in the velocity offset of the [\ion{S}{12}] $\lambda$7609 coronal line & km s$^{-1}$ & float & 1 \\
SXII\_7609\_EQW & Equivalent width of the [\ion{S}{12}] $\lambda$7609 coronal line & \AA\ & float & 1 \\
SXII\_7609\_EQW\_ERR & Error in the equivalent width of the [\ion{S}{12}] $\lambda$7609 coronal line & \AA\ & float & 1 \\
SXII\_7609\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{S}{12}] $\lambda$7609 coronal line & & float & 1 \\
SXII\_7609\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{S}{12}] $\lambda$7609 coronal line & & integer & 1 \\
SXII\_7609\_SKY\_FLAG & Sky line proximity warning for the [\ion{S}{12}] $\lambda$7609 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
SXII\_7609\_NN\_CONF & Neural network confidence level that the [\ion{S}{12}] $\lambda$7609 line is present. & & float & 1 \\
FEX\_6374\_LOGL & Luminosity of the [\ion{Fe}{10}] $\lambda$6374 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEX\_6374\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{10}] $\lambda$6374 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEX\_6374\_FWHM & FWHM of the [\ion{Fe}{10}] $\lambda$6374 coronal line & km s$^{-1}$ & float & 1 \\
FEX\_6374\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{10}] $\lambda$6374 coronal line & km s$^{-1}$ & float & 1 \\
FEX\_6374\_VOFF & Velocity offset of the [\ion{Fe}{10}] $\lambda$6374 coronal line & km s$^{-1}$ & float & 1 \\
FEX\_6374\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{10}] $\lambda$6374 coronal line & km s$^{-1}$ & float & 1 \\
FEX\_6374\_EQW & Equivalent width of the [\ion{Fe}{10}] $\lambda$6374 coronal line & \AA\ & float & 1 \\
FEX\_6374\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{10}] $\lambda$6374 coronal line & \AA\ & float & 1 \\
FEX\_6374\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{10}] $\lambda$6374 coronal line & & float & 1 \\
FEX\_6374\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{10}] $\lambda$6374 coronal line & & integer & 1 \\
FEX\_6374\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{10}] $\lambda$6374 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEX\_6374\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{10}] $\lambda$6374 line is present. & & float & 1 \\
FEVII\_6087\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$6087 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_6087\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$6087 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_6087\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$6087 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_6087\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$6087 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_6087\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$6087 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_6087\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$6087 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_6087\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$6087 coronal line & \AA\ & float & 1 \\
FEVII\_6087\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$6087 coronal line & \AA\ & float & 1 \\
FEVII\_6087\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$6087 coronal line & & float & 1 \\
FEVII\_6087\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$6087 coronal line & & integer & 1 \\
FEVII\_6087\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$6087 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_6087\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$6087 line is present. & & float & 1 \\
FEVII\_5720\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$5720 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5720\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$5720 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5720\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$5720 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5720\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$5720 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5720\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$5720 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5720\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$5720 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5720\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$5720 coronal line & \AA\ & float & 1 \\
FEVII\_5720\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$5720 coronal line & \AA\ & float & 1 \\
FEVII\_5720\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$5720 coronal line & & float & 1 \\
FEVII\_5720\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$5720 coronal line & & integer & 1 \\
FEVII\_5720\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$5720 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_5720\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$5720 line is present. & & float & 1 \\
ARX\_5533\_LOGL & Luminosity of the [\ion{Ar}{10}] $\lambda$5533 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
ARX\_5533\_LOGL\_ERR & Error in the luminosity of the [\ion{Ar}{10}] $\lambda$5533 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
ARX\_5533\_FWHM & FWHM of the [\ion{Ar}{10}] $\lambda$5533 coronal line & km s$^{-1}$ & float & 1 \\
ARX\_5533\_FWHM\_ERR & Error in the FWHM of the [\ion{Ar}{10}] $\lambda$5533 coronal line & km s$^{-1}$ & float & 1 \\
ARX\_5533\_VOFF & Velocity offset of the [\ion{Ar}{10}] $\lambda$5533 coronal line & km s$^{-1}$ & float & 1 \\
ARX\_5533\_VOFF\_ERR & Error in the velocity offset of the [\ion{Ar}{10}] $\lambda$5533 coronal line & km s$^{-1}$ & float & 1 \\
ARX\_5533\_EQW & Equivalent width of the [\ion{Ar}{10}] $\lambda$5533 coronal line & \AA\ & float & 1 \\
ARX\_5533\_EQW\_ERR & Error in the equivalent width of the [\ion{Ar}{10}] $\lambda$5533 coronal line & \AA\ & float & 1 \\
ARX\_5533\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Ar}{10}] $\lambda$5533 coronal line & & float & 1 \\
ARX\_5533\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Ar}{10}] $\lambda$5533 coronal line & & integer & 1 \\
ARX\_5533\_SKY\_FLAG & Sky line proximity warning for the [\ion{Ar}{10}] $\lambda$5533 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
ARX\_5533\_NN\_CONF & Neural network confidence level that the [\ion{Ar}{10}] $\lambda$5533 line is present. & & float & 1 \\
FEVI\_5335\_LOGL & Luminosity of the [\ion{Fe}{6}] $\lambda$5335 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5335\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{6}] $\lambda$5335 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5335\_FWHM & FWHM of the [\ion{Fe}{6}] $\lambda$5335 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5335\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{6}] $\lambda$5335 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5335\_VOFF & Velocity offset of the [\ion{Fe}{6}] $\lambda$5335 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5335\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{6}] $\lambda$5335 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5335\_EQW & Equivalent width of the [\ion{Fe}{6}] $\lambda$5335 coronal line & \AA\ & float & 1 \\
FEVI\_5335\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{6}] $\lambda$5335 coronal line & \AA\ & float & 1 \\
FEVI\_5335\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{6}] $\lambda$5335 coronal line & & float & 1 \\
FEVI\_5335\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{6}] $\lambda$5335 coronal line & & integer & 1 \\
FEVI\_5335\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{6}] $\lambda$5335 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVI\_5335\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{6}] $\lambda$5335 line is present. & & float & 1 \\
CAV\_5309\_LOGL & Luminosity of the [\ion{Ca}{5}] $\lambda$5309 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
CAV\_5309\_LOGL\_ERR & Error in the luminosity of the [\ion{Ca}{5}] $\lambda$5309 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
CAV\_5309\_FWHM & FWHM of the [\ion{Ca}{5}] $\lambda$5309 coronal line & km s$^{-1}$ & float & 1 \\
CAV\_5309\_FWHM\_ERR & Error in the FWHM of the [\ion{Ca}{5}] $\lambda$5309 coronal line & km s$^{-1}$ & float & 1 \\
CAV\_5309\_VOFF & Velocity offset of the [\ion{Ca}{5}] $\lambda$5309 coronal line & km s$^{-1}$ & float & 1 \\
CAV\_5309\_VOFF\_ERR & Error in the velocity offset of the [\ion{Ca}{5}] $\lambda$5309 coronal line & km s$^{-1}$ & float & 1 \\
CAV\_5309\_EQW & Equivalent width of the [\ion{Ca}{5}] $\lambda$5309 coronal line & \AA\ & float & 1 \\
CAV\_5309\_EQW\_ERR & Error in the equivalent width of the [\ion{Ca}{5}] $\lambda$5309 coronal line & \AA\ & float & 1 \\
CAV\_5309\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Ca}{5}] $\lambda$5309 coronal line & & float & 1 \\
CAV\_5309\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Ca}{5}] $\lambda$5309 coronal line & & integer & 1 \\
CAV\_5309\_SKY\_FLAG & Sky line proximity warning for the [\ion{Ca}{5}] $\lambda$5309 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
CAV\_5309\_NN\_CONF & Neural network confidence level that the [\ion{Ca}{5}] $\lambda$5309 line is present. & & float & 1 \\
FEXIV\_5303\_LOGL & Luminosity of the [\ion{Fe}{14}] $\lambda$5303 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEXIV\_5303\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{14}] $\lambda$5303 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEXIV\_5303\_FWHM & FWHM of the [\ion{Fe}{14}] $\lambda$5303 coronal line & km s$^{-1}$ & float & 1 \\
FEXIV\_5303\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{14}] $\lambda$5303 coronal line & km s$^{-1}$ & float & 1 \\
FEXIV\_5303\_VOFF & Velocity offset of the [\ion{Fe}{14}] $\lambda$5303 coronal line & km s$^{-1}$ & float & 1 \\
FEXIV\_5303\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{14}] $\lambda$5303 coronal line & km s$^{-1}$ & float & 1 \\
FEXIV\_5303\_EQW & Equivalent width of the [\ion{Fe}{14}] $\lambda$5303 coronal line & \AA\ & float & 1 \\
FEXIV\_5303\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{14}] $\lambda$5303 coronal line & \AA\ & float & 1 \\
FEXIV\_5303\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{14}] $\lambda$5303 coronal line & & float & 1 \\
FEXIV\_5303\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{14}] $\lambda$5303 coronal line & & integer & 1 \\
FEXIV\_5303\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{14}] $\lambda$5303 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEXIV\_5303\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{14}] $\lambda$5303 line is present. & & float & 1 \\
FEVII\_5276\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$5276 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5276\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$5276 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5276\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$5276 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5276\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$5276 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5276\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$5276 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5276\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$5276 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5276\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$5276 coronal line & \AA\ & float & 1 \\
FEVII\_5276\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$5276 coronal line & \AA\ & float & 1 \\
FEVII\_5276\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$5276 coronal line & & float & 1 \\
FEVII\_5276\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$5276 coronal line & & integer & 1 \\
FEVII\_5276\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$5276 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_5276\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$5276 line is present. & & float & 1 \\
FEVI\_5176\_LOGL & Luminosity of the [\ion{Fe}{6}] $\lambda$5176 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5176\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{6}] $\lambda$5176 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5176\_FWHM & FWHM of the [\ion{Fe}{6}] $\lambda$5176 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5176\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{6}] $\lambda$5176 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5176\_VOFF & Velocity offset of the [\ion{Fe}{6}] $\lambda$5176 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5176\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{6}] $\lambda$5176 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5176\_EQW & Equivalent width of the [\ion{Fe}{6}] $\lambda$5176 coronal line & \AA\ & float & 1 \\
FEVI\_5176\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{6}] $\lambda$5176 coronal line & \AA\ & float & 1 \\
FEVI\_5176\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{6}] $\lambda$5176 coronal line & & float & 1 \\
FEVI\_5176\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{6}] $\lambda$5176 coronal line & & integer & 1 \\
FEVI\_5176\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{6}] $\lambda$5176 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVI\_5176\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{6}] $\lambda$5176 line is present. & & float & 1 \\
FEVII\_5159\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$5159 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5159\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$5159 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_5159\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$5159 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5159\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$5159 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5159\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$5159 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5159\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$5159 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_5159\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$5159 coronal line & \AA\ & float & 1 \\
FEVII\_5159\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$5159 coronal line & \AA\ & float & 1 \\
FEVII\_5159\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$5159 coronal line & & float & 1 \\
FEVII\_5159\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$5159 coronal line & & integer & 1 \\
FEVII\_5159\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$5159 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_5159\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$5159 line is present. & & float & 1 \\
FEVI\_5146\_LOGL & Luminosity of the [\ion{Fe}{6}] $\lambda$5146 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5146\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{6}] $\lambda$5146 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVI\_5146\_FWHM & FWHM of the [\ion{Fe}{6}] $\lambda$5146 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5146\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{6}] $\lambda$5146 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5146\_VOFF & Velocity offset of the [\ion{Fe}{6}] $\lambda$5146 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5146\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{6}] $\lambda$5146 coronal line & km s$^{-1}$ & float & 1 \\
FEVI\_5146\_EQW & Equivalent width of the [\ion{Fe}{6}] $\lambda$5146 coronal line & \AA\ & float & 1 \\
FEVI\_5146\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{6}] $\lambda$5146 coronal line & \AA\ & float & 1 \\
FEVI\_5146\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{6}] $\lambda$5146 coronal line & & float & 1 \\
FEVI\_5146\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{6}] $\lambda$5146 coronal line & & integer & 1 \\
FEVI\_5146\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{6}] $\lambda$5146 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVI\_5146\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{6}] $\lambda$5146 line is present. & & float & 1 \\
FEVII\_4893\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$4893 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_4893\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$4893 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_4893\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$4893 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_4893\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$4893 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_4893\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$4893 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_4893\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$4893 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_4893\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$4893 coronal line & \AA\ & float & 1 \\
FEVII\_4893\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$4893 coronal line & \AA\ & float & 1 \\
FEVII\_4893\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$4893 coronal line & & float & 1 \\
FEVII\_4893\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$4893 coronal line & & integer & 1 \\
FEVII\_4893\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$4893 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_4893\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$4893 line is present. & & float & 1 \\
FEV\_4181\_LOGL & Luminosity of the [\ion{Fe}{5}] $\lambda$4181 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_4181\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{5}] $\lambda$4181 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_4181\_FWHM & FWHM of the [\ion{Fe}{5}] $\lambda$4181 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_4181\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{5}] $\lambda$4181 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_4181\_VOFF & Velocity offset of the [\ion{Fe}{5}] $\lambda$4181 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_4181\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{5}] $\lambda$4181 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_4181\_EQW & Equivalent width of the [\ion{Fe}{5}] $\lambda$4181 coronal line & \AA\ & float & 1 \\
FEV\_4181\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{5}] $\lambda$4181 coronal line & \AA\ & float & 1 \\
FEV\_4181\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{5}] $\lambda$4181 coronal line & & float & 1 \\
FEV\_4181\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{5}] $\lambda$4181 coronal line & & integer & 1 \\
FEV\_4181\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{5}] $\lambda$4181 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEV\_4181\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{5}] $\lambda$4181 line is present. & & float & 1 \\
FEV\_3891\_LOGL & Luminosity of the [\ion{Fe}{5}] $\lambda$3891 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_3891\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{5}] $\lambda$3891 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_3891\_FWHM & FWHM of the [\ion{Fe}{5}] $\lambda$3891 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3891\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{5}] $\lambda$3891 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3891\_VOFF & Velocity offset of the [\ion{Fe}{5}] $\lambda$3891 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3891\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{5}] $\lambda$3891 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3891\_EQW & Equivalent width of the [\ion{Fe}{5}] $\lambda$3891 coronal line & \AA\ & float & 1 \\
FEV\_3891\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{5}] $\lambda$3891 coronal line & \AA\ & float & 1 \\
FEV\_3891\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{5}] $\lambda$3891 coronal line & & float & 1 \\
FEV\_3891\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{5}] $\lambda$3891 coronal line & & integer & 1 \\
FEV\_3891\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{5}] $\lambda$3891 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEV\_3891\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{5}] $\lambda$3891 line is present. & & float & 1 \\
FEV\_3839\_LOGL & Luminosity of the [\ion{Fe}{5}] $\lambda$3839 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_3839\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{5}] $\lambda$3839 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEV\_3839\_FWHM & FWHM of the [\ion{Fe}{5}] $\lambda$3839 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3839\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{5}] $\lambda$3839 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3839\_VOFF & Velocity offset of the [\ion{Fe}{5}] $\lambda$3839 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3839\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{5}] $\lambda$3839 coronal line & km s$^{-1}$ & float & 1 \\
FEV\_3839\_EQW & Equivalent width of the [\ion{Fe}{5}] $\lambda$3839 coronal line & \AA\ & float & 1 \\
FEV\_3839\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{5}] $\lambda$3839 coronal line & \AA\ & float & 1 \\
FEV\_3839\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{5}] $\lambda$3839 coronal line & & float & 1 \\
FEV\_3839\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{5}] $\lambda$3839 coronal line & & integer & 1 \\
FEV\_3839\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{5}] $\lambda$3839 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEV\_3839\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{5}] $\lambda$3839 line is present. & & float & 1 \\
FEVII\_3759\_LOGL & Luminosity of the [\ion{Fe}{7}] $\lambda$3759 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_3759\_LOGL\_ERR & Error in the luminosity of the [\ion{Fe}{7}] $\lambda$3759 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
FEVII\_3759\_FWHM & FWHM of the [\ion{Fe}{7}] $\lambda$3759 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_3759\_FWHM\_ERR & Error in the FWHM of the [\ion{Fe}{7}] $\lambda$3759 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_3759\_VOFF & Velocity offset of the [\ion{Fe}{7}] $\lambda$3759 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_3759\_VOFF\_ERR & Error in the velocity offset of the [\ion{Fe}{7}] $\lambda$3759 coronal line & km s$^{-1}$ & float & 1 \\
FEVII\_3759\_EQW & Equivalent width of the [\ion{Fe}{7}] $\lambda$3759 coronal line & \AA\ & float & 1 \\
FEVII\_3759\_EQW\_ERR & Error in the equivalent width of the [\ion{Fe}{7}] $\lambda$3759 coronal line & \AA\ & float & 1 \\
FEVII\_3759\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Fe}{7}] $\lambda$3759 coronal line & & float & 1 \\
FEVII\_3759\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Fe}{7}] $\lambda$3759 coronal line & & integer & 1 \\
FEVII\_3759\_SKY\_FLAG & Sky line proximity warning for the [\ion{Fe}{7}] $\lambda$3759 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
FEVII\_3759\_NN\_CONF & Neural network confidence level that the [\ion{Fe}{7}] $\lambda$3759 line is present. & & float & 1 \\
NEV\_3426\_LOGL & Luminosity of the [\ion{Ne}{5}] $\lambda$3426 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
NEV\_3426\_LOGL\_ERR & Error in the luminosity of the [\ion{Ne}{5}] $\lambda$3426 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
NEV\_3426\_FWHM & FWHM of the [\ion{Ne}{5}] $\lambda$3426 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3426\_FWHM\_ERR & Error in the FWHM of the [\ion{Ne}{5}] $\lambda$3426 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3426\_VOFF & Velocity offset of the [\ion{Ne}{5}] $\lambda$3426 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3426\_VOFF\_ERR & Error in the velocity offset of the [\ion{Ne}{5}] $\lambda$3426 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3426\_EQW & Equivalent width of the [\ion{Ne}{5}] $\lambda$3426 coronal line & \AA\ & float & 1 \\
NEV\_3426\_EQW\_ERR & Error in the equivalent width of the [\ion{Ne}{5}] $\lambda$3426 coronal line & \AA\ & float & 1 \\
NEV\_3426\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Ne}{5}] $\lambda$3426 coronal line & & float & 1 \\
NEV\_3426\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Ne}{5}] $\lambda$3426 coronal line & & integer & 1 \\
NEV\_3426\_SKY\_FLAG & Sky line proximity warning for the [\ion{Ne}{5}] $\lambda$3426 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
NEV\_3426\_NN\_CONF & Neural network confidence level that the [\ion{Ne}{5}] $\lambda$3426 line is present. & & float & 1 \\
NEV\_3346\_LOGL & Luminosity of the [\ion{Ne}{5}] $\lambda$3346 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
NEV\_3346\_LOGL\_ERR & Error in the luminosity of the [\ion{Ne}{5}] $\lambda$3346 coronal line & $\log(L/$erg s$^{-1})$ & float & 1 \\
NEV\_3346\_FWHM & FWHM of the [\ion{Ne}{5}] $\lambda$3346 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3346\_FWHM\_ERR & Error in the FWHM of the [\ion{Ne}{5}] $\lambda$3346 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3346\_VOFF & Velocity offset of the [\ion{Ne}{5}] $\lambda$3346 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3346\_VOFF\_ERR & Error in the velocity offset of the [\ion{Ne}{5}] $\lambda$3346 coronal line & km s$^{-1}$ & float & 1 \\
NEV\_3346\_EQW & Equivalent width of the [\ion{Ne}{5}] $\lambda$3346 coronal line & \AA\ & float & 1 \\
NEV\_3346\_EQW\_ERR & Error in the equivalent width of the [\ion{Ne}{5}] $\lambda$3346 coronal line & \AA\ & float & 1 \\
NEV\_3346\_F\_FRAC & $\mathcal{F}$ metric of the [\ion{Ne}{5}] $\lambda$3346 coronal line & & float & 1 \\
NEV\_3346\_NPIX & Number of continuous pixels above 3$\sigma$ for the [\ion{Ne}{5}] $\lambda$3346 coronal line & & integer & 1 \\
NEV\_3346\_SKY\_FLAG & Sky line proximity warning for the [\ion{Ne}{5}] $\lambda$3346 coronal line. True if within 20 \AA\ of 5578.5, 5894.6, 6301.7, or 7246.0 in the observed frame. & & boolean & 1 \\
NEV\_3346\_NN\_CONF & Neural network confidence level that the [\ion{Ne}{5}] $\lambda$3346 line is present. & & float & 1 \\
ARIII\_7135\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
ARIII\_7135\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
ARIII\_7135\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
ARIII\_7135\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
ARIII\_7135\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
ARIII\_7135\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
ARIII\_7135\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
ARIII\_7135\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
ARIII\_7135\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
ARIII\_7135\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
SII\_6731\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6731\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6731\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
SII\_6731\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
SII\_6731\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
SII\_6731\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
SII\_6731\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6731\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6731\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
SII\_6731\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
SII\_6717\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6717\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6717\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
SII\_6717\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
SII\_6717\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
SII\_6717\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
SII\_6717\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6717\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
SII\_6717\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
SII\_6717\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
NII\_6584\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6584\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6584\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
NII\_6584\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NII\_6584\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
NII\_6584\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NII\_6584\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6584\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6584\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
NII\_6584\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
H\_ALPHA\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_ALPHA\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_ALPHA\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
H\_ALPHA\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_ALPHA\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
H\_ALPHA\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_ALPHA\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_ALPHA\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_ALPHA\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
H\_ALPHA\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
NII\_6548\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6548\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6548\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
NII\_6548\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NII\_6548\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
NII\_6548\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NII\_6548\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6548\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
NII\_6548\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
NII\_6548\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OI\_6302\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OI\_6302\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OI\_6302\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OI\_6302\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OI\_6302\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OI\_6302\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OI\_6302\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OI\_6302\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OI\_6302\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OI\_6302\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
HEI\_5876\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
HEI\_5876\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
HEI\_5876\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
HEI\_5876\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
HEI\_5876\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
HEI\_5876\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
HEI\_5876\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
HEI\_5876\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
HEI\_5876\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
HEI\_5876\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OIII\_5007\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_5007\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_5007\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_5007\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_5007\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_5007\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_5007\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_5007\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_5007\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OIII\_5007\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OIII\_4959\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4959\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4959\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_4959\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_4959\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_4959\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_4959\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4959\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4959\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OIII\_4959\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
H\_BETA\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_BETA\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_BETA\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
H\_BETA\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_BETA\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
H\_BETA\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_BETA\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_BETA\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_BETA\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
H\_BETA\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OIII\_4363\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4363\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4363\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_4363\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_4363\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OIII\_4363\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OIII\_4363\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4363\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OIII\_4363\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OIII\_4363\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
H\_GAMMA\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_GAMMA\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_GAMMA\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
H\_GAMMA\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_GAMMA\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
H\_GAMMA\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_GAMMA\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_GAMMA\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_GAMMA\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
H\_GAMMA\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
H\_DELTA\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_DELTA\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_DELTA\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
H\_DELTA\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_DELTA\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
H\_DELTA\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
H\_DELTA\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_DELTA\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
H\_DELTA\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
H\_DELTA\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
NEIII\_3869\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
NEIII\_3869\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
NEIII\_3869\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
NEIII\_3869\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NEIII\_3869\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
NEIII\_3869\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
NEIII\_3869\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
NEIII\_3869\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
NEIII\_3869\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
NEIII\_3869\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OII\_3729\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3729\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3729\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OII\_3729\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OII\_3729\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OII\_3729\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OII\_3729\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3729\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3729\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OII\_3729\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
OII\_3726\_CONT & Continuum luminosity at the line center from 200-pixel median smoothing of the line-subtracted spectrum & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3726\_CONT\_ERR & Error in the continuum luminosity & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3726\_EQW & Equivalent width of the emission line, accounting for stellar absorption & \AA\ & float & 3  \\
OII\_3726\_EQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OII\_3726\_REQW & Equivalent width of the emission line, not accounting for stellar absorption & \AA\ & float & 3  \\
OII\_3726\_REQW\_ERR & Error in the equivalent width of the emission line & \AA\ & float & 3 \\
OII\_3726\_LOGL & Luminosity of the emission line from a Gaussian fit & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3726\_LOGL\_ERR & Error in the luminosity of the emission line & $\log(L/$erg s$^{-1})$ & float & 3 \\
OII\_3726\_INST\_RES & Instrumental resolution at the line center & km s$^{-1}$ & float & 3 \\
OII\_3726\_CHISQ & Reduced $\chi^2$ of the line fit used in the EQW measurements & & float & 3 \\
\enddata
\begin{tablenotes}
    \item[0] Source references:
    \item[1] [1] this work
    \item[2] [2] SDSS
    \item[3] [3] MPA/JHU
    \item[4] [4] AllWISE
    \item[5] [5] NSA
\end{tablenotes}
\end{deluxetable*}
